Influence Pathway Discovery on Social Media

This paper addresses influence pathway discovery, a key emerging problem in today's online media. We propose a discovery algorithm that leverages recently published work on unsupervised interpretable ideological embedding, a mapping of ideological beliefs (done in a self-supervised fashion) into interpretable low-dimensional spaces. Computing the ideological embedding at scale allows one to analyze correlations between the ideological positions of leaders, influencers, news portals, or population segments, deriving potential influence pathways. The work is motivated by the importance of social media as the preeminent means for global interactions and collaborations on today's Internet, as well as their frequent (mis-)use to wield influence that targets social beliefs and attitudes of selected populations. Tools that enable the understanding and mapping of influence propagation through population segments on social media are therefore increasingly important. In this paper, influence is measured by the perceived ideological shift over time that is correlated with influencers' activity. Correlated shifts in ideological embeddings indicate changes, such as swings/switching (among competing ideologies), polarization (depletion of neutral ideological positions), escalation/radicalization (shifts to more extreme versions of the ideology), or unification/cooldown (shifts towards more neutral stances). Case-studies are presented to explore selected influence pathways (i) in a recent French election, (ii) during political discussions in the Philippines, and (iii) for some Russian messaging during the Russia/Ukraine conflict.

==> implementation.tex <==

\subsection{Pipeline implementation}
%%\comment{Ruijie}
We have employed a robust and versatile tech stack to deliver a dynamic and efficient solution. On the frontend, we leveraged the power of React JS, allowing us to create a responsive and interactive operator interface that seamlessly adapts to operator actions. On the backend, Django has been the cornerstone of our operations, providing a secure and scalable framework for handling data, logic, and server-side operations. To store and manage our data, we opted for MongoDB, harnessing the flexibility and scalability of a NoSQL database. Furthermore, we streamlined our deployment and containerization processes by dockerizing the entire system, ensuring consistency and ease of scaling across various environments. The overall framework is shown in Figure~\ref{fig:development}, and we implemented the following key features:
%This tech stack combination has enabled us to create a robust and high-performance application that meets our project's requirements effectively. 
\begin{enumerate}
    \item \textbf{Influence network}: We visualized the derived influence networks using the react-vis-network-graph library, illustrating the influence propagation within the network;
    \item \textbf{Influence heatmap}: We incorporated a heatmap graph using the Plotly library, quantitatively displays the Pearson-correlation between each pair of entities;
    \item \textbf{Ideology time-series}: We integrated a time-series graph utilizing the Plotly library to enable a comparison of ideology trends and shifts  between entity pairs within the influence graph over time;
    %allowing us to track and analyze ideological trends and shifts;
    \item \textbf{Detailed information}: This feature provides operators with the detailed information about each entity within the influence graph;  
    %can access comprehensive node data, enhancing their understanding of the network's components and their respective attributes;
    \item \textbf{Entity selection bar}: This feature serves as a central hub for operators to manage views and entity selection within the influence graph. 
    %Operators can easily control and customize their graph experience by selecting and manipulating nodes and views, enhancing their ability to explore and interact with the network data.
\end{enumerate}
